Beyond the Selected Completely At Random Assumption for Learning from Positive and Unlabeled Data

Most positive and unlabeled data is subject to selection biases. The labeled examples can, for example, be selected from the positive set because they are easier to obtain or more obviously positive. This paper investigates how learning can be ena BHbled in this setting. We propose and theoretically analyze an empirical-risk-based method for incorporating the labeling mechanism. Additionally, we investigate under which assumptions learning is possible when the labeling mechanism is not fully understood and propose a practical method to enable this. Our empirical analysis supports the theoretical results and shows that taking into account the possibility of a selection bias, even when the labeling mechanism is unknown, improves the trained classifiers.

==> ydocincl.tex <==
%%
%% This is file `ydocincl.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% ydoc.dtx  (with options: `ydocincl.tex')
%% 
\expandafter\ifx\csname ydocinclversion\endcsname\relax\else
    \endinput
\fi

\chardef\ydocinclversion=1

\newread\inFile
\newread\subFile
\newwrite\outFile
\newif\ifContinue
\newlinechar=`^^J

\def\makeOther#1{\catcode`#1=12\relax}

\let\inLine\relax
\let\lastLine\relax

\def\includefiles#1#2{%
    \begingroup
    \immediate\openin\inFile#1\relax
    \immediate\openout\outFile#2\relax
    \makeOther\@%
    \makeOther\ \makeOther\\\makeOther\$%
    \makeOther\#\makeOther\^\makeOther\^^K%
    \makeOther\_\makeOther\^^A\makeOther\%%
    \makeOther\~\makeOther\{\makeOther\}\makeOther\&%
    \endlinechar-1\relax
    \Continuetrue
    \loop
      \let\lastLine\inLine
      \read\inFile to\inLine
      \ifeof\inFile
        \Continuefalse
      \else
        \expandafter\checkLine\inLine\empty\empty\empty\endLine
      \fi
      \ifContinue
    \repeat
    \immediate\closein\inFile
    \immediate\closeout\outFile
    \endgroup
    \end
}

\def\copyline{%
    \immediate\write\outFile{\inLine}%
}

\chardef\percentcharnum=`\%

\begingroup
\makeOther\%\makeOther\@\relax
\gdef\SubFileOptionString{%<@}\relax
\gdef\CommentChar{%}\relax
\catcode`\|=0
\makeOther\ \makeOther\\|relax
|gdef|IfFalseString{% \iffalse}|relax
|gdef|FiString{% \fi}|relax
|endgroup

\def\checkLine#1#2#3#4\endLine{%
    \def\firstthree{#1#2#3}%
    \ifx\firstthree\SubFileOptionString
        \readSubFile#4\endLine
    \else
        \copyline
    \fi
}

\def\readSubFile#1>#2\endLine{%
    \immediate\openin\subFile=#1\relax
    \ifeof\subFile
        % File not found
    \else
        \message{^^JIncluding subfile '#1'^^J}%
        \immediate\write\outFile{\CommentChar<*#1>}%
        \ifx\lastLine\IfFalseString
            \immediate\write\outFile{\FiString}%
        \fi
        \copySubFile
        \ifx\lastLine\IfFalseString
            \immediate\write\outFile{\IfFalseString}%
        \fi
        \immediate\write\outFile{\CommentChar</#1>}%
    \fi
    \immediate\closein\subFile
}

\def\copySubFile{%
    \read\subFile to\subLine
    \ifeof\subFile\else
        \immediate\write\outFile{\subLine}%
        \expandafter\copySubFile
    \fi
}
\endinput
%%
%% End of file `ydocincl.tex'.


==> ydocstrip.tex <==
%%
%% This is file `ydocstrip.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% ydoc.dtx  (with options: `ydocstrip.tex')
%% 
\expandafter\ifx\csname ydocstripversion\endcsname\relax\else
    \endinput
\fi

\chardef\ydocstripversion=1

\input docstrip

\def\checkOption<#1{%
  \ifcase
    \ifx*#10\else \ifx/#11\else
    \ifx+#12\else \ifx-#13\else
    \ifx<#14\else
    \ifx=#15\else
    \ifx!#16\else
    10\fi\fi\fi\fi\fi\fi\fi\relax
  \expandafter\starOption\or
  \expandafter\slashOption\or
  \expandafter\plusOption\or
  \expandafter\minusOption\or
  \expandafter\verbOption\or
  \expandafter\varOption\or
  \expandafter\valueOption\else
  \expandafter\doOption\fi
  #1}

\def\varOption =#1#2>#3\endLine{{%
    \ifx*#1\relax
        \edef\varStop{\perCent<=/#2>}%
        \global\expandafter\let\csname ydocstrip@var@#2\endcsname\empty%
        \expandafter\def\csname ydocstrip@var@#2\endcsname##1{}%
        \loop
            \ifeof\inFile
                \errmessage{Source file ended while reading a multi-line variable content!}%
            \fi
            \read\inFile to \inLine
        \if 1\ifx\inLine\varStop 0\fi 1% if not inLine==varStop
            \expandafter\xdef\csname ydocstrip@var@#2\endcsname{\csname ydocstrip@var@#2\endcsname^^J\inLine}%
            \maybeMsg{.}%
        \repeat
    \else
    \ifx/#1\relax
        \errmessage{Error in expression: spurious '<=/#2>'}%
    \else
    \ifx+#1\relax
        \expandafter\ifx\csname ydocstrip@var@#2\endcsname\relax
            \expandafter\xdef\csname ydocstrip@var@#2\endcsname{#3}%
        \else
            \expandafter\xdef\csname ydocstrip@var@#2\endcsname{\csname ydocstrip@var@#2\endcsname^^J#3}%
        \fi
    \else
        \expandafter\gdef\csname ydocstrip@var@#1#2\endcsname{#3}%
    \fi
    \fi
    \fi
}}

\def\valueOption !#1>#2\endLine{%
    \begingroup
    \expandafter\let\expandafter\var\csname ydocstrip@var@#1\endcsname
    \ifx\var\relax
        \errmessage{Used variable '#1' was never defined!}%
    \else
    \ifx\var\empty\else
        \def\do##1##2##3{%
            \StreamPut##1{\csname ydocstrip@var@#1\endcsname}%
        }%
        \activefiles
    \fi
    \fi
    \endgroup
}
\endinput
%%
%% End of file `ydocstrip.tex'.

